Self-Review Reinforcement Learning (SRRL) with Cross-Episode Memory and Policy Distillation

Reinforcement Learning is commonly used to train large language models using environmental feedback. In applied settings, the environment usually provides sparse or delayed feedback. This makes it difficult for the model to pinpoint which actions in its reasoning led to success or failure. So, learning effectively from these signals is hard because the model must determine how each failure should inform meaningful behavioral corrections in subsequent iterations. We introduce a training framework, Self-Review Reinforcement Learning, that embeds an explicit self-review step into each RL episode. When a first-pass response fails, the model generates a self-review to identify what went wrong, which conditions an improved second attempt. Unlike inference-time reflection approaches, such as Reflexion, the framework optimizes self-review with policy gradients and internalizes improvements into the base policy via selective distillation, ensuring they persist across future episodes. A cross-episode memory keeps successful self-reviews for reuse when encountering similar tasks in future episodes during training. We evaluate SRRL against a standard RLVR baseline using the GRPO optimizer across two language models, Qwen 3-4B and OLMo-3- 7B, on GSM8K benchmark. SRRL consistently outperforms the RLVR in final reward performance and achieves greater learning efficiency by successfully transforming feedback into behavioral improvement.

==> erl.tex <==

\begin{tikzpicture}[
  font=\small,
  >={Stealth[length=1mm]},
  box/.style={draw, rounded corners, align=left, minimum height=9mm, inner sep=3.5pt, line width=0.75pt},
  wide/.style={box, minimum width=25mm},
  med/.style={box, minimum width=20mm},
  small/.style={box, minimum width=10mm},
  note/.style={font=\small, inner sep=2pt},
line/.style={-Stealth, line width=2pt},
]

% ------------------ TOP ROW ------------------
\node[small] (task) {Task $x$};

\node[wide, right=14mm of task] (pi1)
{Policy $\pi_\theta$\\\textit{Attempt 1}};

\node[med, right=14mm of pi1] (env1)
{Environment\\Feedback $f$\\Outcome $r$};

\node[wide, right=14mm of env1] (ref)
{Review + Compare\\
$\mathrm{cmp}(y^{(1)}, f, \mathcal{M})$};

\node[small, right=14mm of ref] (delta)
{Plan $\Delta$};

\node[wide, right=16mm of delta] (pi2)
{Policy $\pi_\theta(\cdot|\Delta)$\\\textit{Attempt 2}};

\node[med, right=14mm of pi2] (env2)
{Environment\\Outcome $r'$};

\draw[line] (task) -- (pi1);
\draw[line] (pi1) -- node[note, above] {$y^{(1)}$} (env1);
\draw[line] (env1) -- node[note, above] {$f, r$} (ref);
\draw[line] (ref) -- node[note, above] {$\Delta$} (delta);
\draw[line] (delta) -- (pi2);
\draw[line] (pi2) -- node[note, above] {$y^{(2)}$} (env2);

\node[note, above=4mm of pi1] {First-Pass Response (RL)};
\node[note, above=4mm of ref] {Self-Review + Memory};
\node[note, above=4mm of pi2] {Second-Pass Response (RL)};

% ------------------ BOTTOM ROW ------------------
\node[wide, below=18mm of env1, minimum width=52mm] (mem)
{Cross-episode memory $\mathcal{M}$\\\textit{(strategies, traces, mistakes)}};

\node[small, below=15mm of delta] (rdelta)
{Credit $r_\Delta$};

\node[wide, below=45mm of pi2, minimum width=40mm] (update)
{Policy update (RL)\\
$r_{\text{total}} = r' + \lambda r_\Delta$};

\node[wide, left=30mm of update, minimum width=50mm] (distill)
{Internalize (SFT / distill)\\
$\pi_\theta \leftarrow \pi_\theta(\cdot|\Delta)$};

\node[note, above=4mm of distill] {Consolidation};

% Define clean "ports" on update for inputs
\coordinate (updateN) at ($(update.north)+(0,0)$);
\coordinate (updateS) at ($(update.south)+(0,0)$);

% Memory retrieve/store (short orthogonal, no crossing)
\draw[line]
(mem.north) -- ++(0,7mm) -|
node[note, pos=0.85, right=-13mm] {retrieve}
(ref.south);

\draw[line]
(ref.south) -- ++(0,-7mm) -|
node[note, pos=0.85, left=-10mm] {store}
(mem.north);

% Reflection credit: ref -> rdelta (vertical)
\draw[line] (ref.south) -- node[note, right] {$r_\Delta$} (rdelta.north);

% Outcome r' : env2 -> updateN (vertical)  (no diagonals)
\draw[line] (env2.south) -- node[note, right] {$r'$} (updateN);

% Credit rΔ : route UNDER update, then enter at updateS (avoids side crowding)
\draw[line] (rdelta.south) -- node[note, midway, right] {$r_\Delta$} (updateN);

% Update -> distill (straight)
\draw[line] (update.west) -- (distill.east);

% Small deployment note (kept, but not crossing)
\node[note, below=2mm of pi1] {(\textit{base policy used at deployment})};

% Place persistence note BELOW consolidation lane (no overlap)
\node[note, below=3mm of distill] {};

\end{tikzpicture}

